The impact of (n,$\gamma$) reaction rate uncertainties on the predicted abundances of i-process elements with $32\leq Z\leq 48$ in the metal-poor star HD94028

Several anomalous elemental abundance ratios have been observed in the metal-poor star HD94028. We assume that its high [As/Ge] ratio is a product of a weak intermediate (i) neutron-capture process. Given that observational errors are usually smaller than predicted nuclear physics uncertainties, we have first set up a benchmark one-zone i-process nucleosynthesis simulation results of which provide the best fit to the observed abundances. We have then performed Monte Carlo simulations in which 113 relevant (n,$\gamma$) reaction rates of unstable species were randomly varied within Hauser-Feshbach model uncertainty ranges for each reaction to estimate the impact on the predicted stellar abundances. One of the interesting results of these simulations is a double-peaked distribution of the As abundance, which is caused by the variation of the $^{75}$Ga (n,$\gamma$) cross section. This variation strongly anti-correlates with the predicted As abundance, confirming the necessity for improved theoretical or experimental bounds on this cross section. The $^{66}$Ni (n,$\gamma$) reaction is found to behave as a major bottleneck for the i-process nucleosynthesis. Our analysis finds the Pearson product-moment correlation coefficient $r_\mathrm{P} > 0.2$ for all of the i-process elements with $32 \leq Z \leq 42$, with significant changes in their predicted abundances showing up when the rate of this reaction is reduced to its theoretically constrained lower bound. Our results are applicable to any other stellar nucleosynthesis site with the similar i-process conditions, such as Sakurai's object (V4334 Sagittarii) or rapidly-accreting white dwarfs.

==> vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\nabla \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
% end vectors.tex

